Towards Automatic Model Comparison: An Adaptive Sequential Monte Carlo Approach

Model comparison for the purposes of selection, averaging and validation is a problem found throughout statistics. Within the Bayesian paradigm, these problems all require the calculation of the posterior probabilities of models within a particular class. Substantial progress has been made in recent years, but difficulties remain in the implementation of existing schemes. This paper presents adaptive sequential Monte Carlo (\smc) sampling strategies to characterise the posterior distribution of a collection of models, as well as the parameters of those models. Both a simple product estimator and a combination of \smc and a path sampling estimator are considered and existing theoretical results are extended to include the path sampling variant. A novel approach to the automatic specification of distributions within \smc algorithms is presented and shown to outperform the state of the art in this area. The performance of the proposed strategies is demonstrated via an extensive empirical study. Comparisons with state of the art algorithms show that the proposed algorithms are always competitive, and often substantially superior to alternative techniques, at equal computational cost and considerably less application-specific implementation effort.

==> tab/gmm-bf.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lCCCC}
      \toprule
      Proposal scales  & \multicolumn{2}{c}{Manual} & Adaptive & Automatic \\
      \cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
      Annealing scheme & Prior (2) & \multicolumn{3}{c}{Adaptive} \\
      \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-5}
      Algorithm   & \multicolumn{4}{c}{Bayes facor estimates ($\log B_{4,5}\pm\text{\sd}$)} \\ \midrule
      \smctwo-\ds & $2.15\pm0.25$ & $2.14\pm0.21$ & $\B2.15\pm0.19$ & $2.15\pm0.20$ \\
      \smctwo-\ps & $2.15\pm0.23$ & $2.15\pm0.20$ & $\R2.15\pm0.18$ & $2.15\pm0.21$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
\end{table}


==> tab/node-c-all.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{llllCCC}
      \toprule
      &&&& \multicolumn{2}{c}{Marginal likelihood ($\log p(\paramk|\data)\pm\text{\sd})$} & \\ \cmidrule(lr){5-6}
      $T$ & Proposal Scales & Annealing scheme & Algorithm & $m = 3$ & $m = 5$ & Bayes factor $\log B_{5,3}$ \\ \midrule
      $10 $ & Manual    & Prior (5) & \pmcmc      & $-1651.0\pm27.9$   & $-85.1\pm36.6$   & $1565.9\pm42.1$ \\
      $30 $ &           &           &             & $\B-1639.7\pm7.4$  & $\B-78.9\pm11.2$ & $\B1560.8\pm12.8$ \\
      $100$ &           &           &             & $-1624.6\pm15.7$   & $-75.7\pm24.8$   & $1548.9\pm25.6$ \\ \midrule
      $500$ & Manual    & Prior (5) & \smctwo-\ds & $-1640.7\pm10.8$   & $-78.5\pm9.8$    & $1562.2\pm10.1$ \\
            &           &           & \smctwo-\ps & $-1640.8\pm 8.4$   & $-79.2\pm7.9$    & $1561.6\pm 8.5$ \\
      $500$ & Manual    & Adaptive  & \smctwo-\ds & $-1639.7\pm 6.9$   & $-78.6\pm4.8$    & $1561.1\pm7.1$ \\
            &           &           & \smctwo-\ps & $-1640.1\pm 5.4$   & $-78.8\pm3.7$    & $1561.3\pm6.8$ \\
      $500$ & Adaptive  & Adaptive  & \smctwo-\ds & $-1639.8\pm 2.2$   & $-79.4\pm1.7$    & $1560.4\pm3.1$ \\
            &           &           & \smctwo-\ps & $\R-1640.2\pm 1.9$ & $\R-78.5\pm1.5$  & $\R1561.7\pm2.3$ \\
      $500$ & Automatic & Adaptive  & \smctwo-\ds & $-1640.7\pm 2.8$   & $-79.2\pm2.2$    & $1561.5\pm3.8$ \\
            &           &           & \smctwo-\ps & $\R-1640.1\pm 2.5$ & $-78.9\pm2.0$    & $1561.2\pm3.7$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Results for non-linear \ode models with data generated from complex
    model. {\B Italic}: Best for the same algorithm, proposal scales
    and annealing scheme. {\R Bold}: Best for all samplers.}
  \label{tab:node-c-all}
\end{table}


==> tab/node-c.tex <==
\begin{table}
  \begingroup\small\begin{tabularx}{\linewidth}{llXXX}
    \toprule
    & & \multicolumn{2}{c}{Marginal likelihood} & \\
    \cmidrule(lr){3-4}
    Algorithm & $T$ & $m = 3$ & $m = 5$ & Bayes factor $B_{3,5}$ \\
    \midrule
    \pmcmc & $10 $ & $-1651.0\pm27.9$             & $-85.1\pm36.6$             & $1565.9\pm42.1$ \\
           & $30 $ & $\color{blue}\it -1639.7\pm 7.4$ & $\color{blue}\it -78.9\pm11.2$ & $\color{blue}\it 1560.8\pm12.8$ \\
           & $100$ & $-1624.6\pm15.7$             & $-75.7\pm24.8$             & $1548.9\pm25.6$ \\
    \midrule
    \smctwo-\ds & $500$ & $-1640.7\pm10.8$            & $-78.5\pm9.8$            & $1562.2\pm10.1$ \\
    \smctwo-\ps & $500$ & $\color{red}\bf -1640.8\pm 8.4$ & $\color{red}\bf -79.2\pm7.9$ & $\color{red}\bf 1561.6\pm 8.5$ \\
    \bottomrule
  \end{tabularx}\endgroup
  \caption{Results for non-linear \ode models with data generated from complex
    model}
  \label{tab:node-complex}
\end{table}


==> tab/node-s-all.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{llllccc}
      \toprule
      &&&& \multicolumn{2}{c}{Marginal likelihood ($\log p(\paramk|\data)\pm\text{\sd})$} & \\ \cmidrule(lr){5-6}
      $T$ & Proposal Scales & Annealing scheme & Algorithm & $m = 3$ & $m = 5$ & Bayes factor $\log B_{3,5}$ \\ \midrule
      $10 $ & Manual    & Prior (5) & \pmcmc      & $-109.7\pm3.2$   & $-120.3\pm2.5$   & $10.6\pm3.8$ \\
      $30 $ &           &           &             & $\B-105.0\pm1.2$ & $\B-116.1\pm2.2$ & $\B11.2\pm2.5$ \\
      $100$ &           &           &             & $-134.7\pm7.9$   & $-144.1\pm6.2$   & $9.4\pm11.2$ \\ \midrule
      $500$ & Manual    & Prior (5) & \smctwo-\ds & $-104.6\pm2.0$   & $-112.7\pm1.8$   & $8.1\pm2.8$ \\
            &           &           & \smctwo-\ps & $-104.5\pm1.8$   & $-112.7\pm1.5$   & $8.2\pm2.5$ \\
      $500$ & Manual    & Adaptive  & \smctwo-\ds & $-104.5\pm1.1$   & $-112.7\pm1.1$   & $8.1\pm1.6$ \\
            &           &           & \smctwo-\ps & $-104.6\pm1.0$   & $-112.8\pm1.0$   & $8.2\pm1.5$ \\
      $500$ & Adaptive  & Adaptive  & \smctwo-\ds & $-104.5\pm0.5$   & $-112.7\pm0.4$   & $8.1\pm0.8$ \\
            &           &           & \smctwo-\ps & $\R-104.6\pm0.4$ & $\R-112.8\pm0.3$ & $\R8.1\pm0.6$ \\
      $500$ & Automatic & Adaptive  & \smctwo-\ds & $-104.5\pm0.8$   & $-112.7\pm0.6$   & $8.1\pm1.2$ \\
            &           &           & \smctwo-\ps & $-104.6\pm0.7$   & $-112.7\pm0.5$   & $8.1\pm1.1$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Results for non-linear \ode models with data generated from simple
    model. {\B italic}: Best for the same algorithm. {\R Bold}: Best for all
    samplers.}
  \label{tab:node-s-all}
\end{table}


==> tab/node-s.tex <==
\begin{table}
  \begingroup\small\begin{tabularx}{\linewidth}{llXXX}
    \toprule
    & & \multicolumn{2}{c}{Marginal likelihood} & \\
    \cmidrule(lr){3-4}
    Algorithm & $T$ & $m = 3$ & $m = 5$ & Bayes factor $B_{3,5}$ \\
    \midrule
    \pmcmc & $10 $ & $-109.7\pm3.2$             & $-120.3\pm2.5$             & $10.6\pm3.8$ \\
           & $30 $ & $\color{blue}\it -105.0\pm1.2$ & $\color{blue}\it -116.1\pm2.2$ & $\color{blue}\it 11.2\pm2.5$ \\
           & $100$ & $-134.7\pm7.9$             & $-144.1\pm6.2$             & $9.4\pm11.2$ \\
    \midrule
    \smctwo-\ds & $500$ & $-104.6\pm2.0$            & $-112.7\pm1.8$            & $8.1\pm2.8$ \\
    \smctwo-\ps & $500$ & $\color{red}\bf-104.5\pm1.8$ & $\color{red}\bf-112.7\pm1.5$ & $\color{red}\bf8.2\pm2.5$ \\
    \bottomrule
  \end{tabularx}\endgroup
  \caption{Results for non-linear \ode models with data generated from complex
    model}
  \label{tab:node-simple}
\end{table}


==> tab/pet-bf-par-all.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lllCCCCCCCC}
      \toprule
      \multicolumn{3}{l}{Proposal scales}  & \multicolumn{6}{c}{Manual} & Adaptive & Automatic \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-9}\cmidrule(lr){10-10}\cmidrule(lr){11-11}
      \multicolumn{3}{l}{Annealing scheme} & Linear & Prior (2) & Prior (5) & Posterior (2) & Posterior (5) & \multicolumn{3}{c}{Adaptive} \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-11}
      %
      $T$    & $N$   & Algorithm   & \multicolumn{8}{c}{Bayes facor estimates ($\log B_{2,1}\pm\text{\sd}$)} \\ \midrule
      $500$  & $30 $ & \pmcmc      & $-16.4\pm117.20$ & $  1.5\pm  4.13$ & $  1.7\pm  0.62$ & $-23.8\pm229.67$ & $-70.9\pm525.79$ &&& \\
      $500$  & $192$ & \smctwo-\ds & $\B1.6\pm0.33$ & $\B1.6\pm0.28$ & $\B1.6\pm0.27$ & $\B1.4\pm0.62$ & $\B1.3\pm1.13$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
             &       & \smctwo-\ps & $0.2\pm6.68$   & $\B1.6\pm0.28$ & $\B1.6\pm0.27$ & $0.1\pm11.50$  & $-3.9\pm30.02$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
      $100 $ & $960$ & \smctwo-\ds & $1.4\pm0.59$   & $1.6\pm0.38$   & $1.6\pm0.37$   & $1.3\pm1.10$   & $0.5\pm1.55$    & $1.6\pm0.34$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\
             &       & \smctwo-\ps & $-1.3\pm13.36$ & $1.5\pm0.43$   & $1.6\pm0.37$   & $-4.7\pm23.79$ & $-13.1\pm66.30$ & $1.6\pm0.33$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\ \midrule
      $1000$ & $30 $ & \pmcmc      & $ -2.9\pm 99.47$ & $  1.4\pm  3.08$ & $  1.6\pm  0.49$ & $-12.0\pm183.78$ & $-67.3\pm400.21$ &&& \\
      $1000$ & $192$ & \smctwo-\ds & $\B1.6\pm0.24$ & $\B1.6\pm0.17$ & $\B1.6\pm0.21$ & $\B1.6\pm0.42$ & $\B1.5\pm0.79$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.14$ \\
             &       & \smctwo-\ps & $1.0\pm2.38$   & $\B1.6\pm0.17$ & $\B1.6\pm0.21$ & $1.4\pm5.65$   & $-0.6\pm15.47$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.13$ \\
      $200 $ & $960$ & \smctwo-\ds & $1.6\pm0.39$   & $1.6\pm0.24$   & $1.6\pm0.25$   & $1.5\pm0.58$   & $1.1\pm1.25$    & $1.6\pm0.19$   & $1.6\pm0.12$   & $1.6\pm0.13$ \\
             &       & \smctwo-\ps & $-0.9\pm7.51$  & $1.6\pm0.23$   & $1.6\pm0.24$   & $-1.1\pm12.20$ & $-11.7\pm34.68$ & $\B1.6\pm0.18$ & $\R1.6\pm0.11$ & $\B1.6\pm0.12$ \\ \midrule
      $2000$ & $30 $ & \pmcmc      & $-14.3\pm 60.88$ & $  0.8\pm  1.99$ & $  1.6\pm  0.31$ & $-14.7\pm132.57$ & $-95.5\pm264.74$ &&& \\
      $2000$ & $192$ & \smctwo-\ds & $\B1.6\pm0.18$ & $\B1.6\pm0.13$ & $\B1.6\pm0.14$ & $\B1.6\pm0.24$ & $\B1.6\pm0.44$  & $1.6\pm0.13$   & $1.6\pm0.09$   & $1.6\pm0.11$ \\
             &       & \smctwo-\ps & $1.6\pm1.34$   & $\B1.6\pm0.13$ & $\B1.6\pm0.14$ & $1.6\pm2.98$   & $1.6\pm6.06$    & $1.6\pm0.13$   & $1.7\pm0.09$   & $1.6\pm0.10$ \\
      $400 $ & $960$ & \smctwo-\ds & $\B1.6\pm0.18$ & $1.6\pm0.14$   & $1.6\pm0.16$   & $1.6\pm0.32$   & $1.5\pm0.74$    & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\
             &       & \smctwo-\ps & $0.5\pm3.15$   & $1.6\pm0.14$   & $1.6\pm0.16$   & $0.1\pm6.77$   & $-4.2\pm17.15$  & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\ \midrule
      $5000$ & $30$  & \pmcmc      & $-14.0\pm 42.91$ & $  1.2\pm  1.32$ & $  1.6\pm  0.24$ & $-27.9\pm 73.39$ & $-60.3\pm198.10$ &&& \\
      $5000$ & $192$ & \smctwo-\ds & $1.6\pm0.13$   & $1.6\pm0.10$   & $1.6\pm0.10$   & $\B1.6\pm0.17$ & $\B1.6\pm0.23$  & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
             &       & \smctwo-\ps & $1.6\pm0.64$   & $1.6\pm0.10$   & $1.6\pm0.10$   & $1.5\pm1.26$   & $1.3\pm2.98$    & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
      $1000$ & $960$ & \smctwo-\ds & $\B1.6\pm0.11$ & $\B1.6\pm0.08$ & $\B1.6\pm0.09$ & $\B1.6\pm0.17$ & $1.6\pm0.33$    & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $1.6\pm0.06$ \\
             &       & \smctwo-\ps & $1.2\pm1.32$   & $\B1.6\pm0.08$ & $\B1.6\pm0.09$ & $0.6\pm2.48$   & $-0.2\pm6.63$   & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $\B1.6\pm0.05$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Bayes factor $B_{2,1}$ estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. The \pmcmc and \smc with $N = 192$ are completely $N$-way
    parallelized.  \smc with $N = 960$ are $N/5$-way parallelized. {\B
      Italic}: Best for the same computational cost and the same schedule.
    {\R Bold}: Best for the same computaitonal cost and all schedules.}
  \label{tab:pet-bf-par-all}
\end{table}


% & $-16.4\pm117.20$ & $  1.5\pm  4.13$ & $  1.7\pm  0.62$ & $-23.8\pm229.67$ & $-70.9\pm525.79$ &&& \\
% & $\B1.6\pm0.33$ & $\B1.6\pm0.28$ & $\B1.6\pm0.27$ & $\B1.4\pm0.62$ & $\B1.3\pm1.13$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
% & $0.2\pm6.68$   & $\B1.6\pm0.28$ & $\B1.6\pm0.27$ & $0.1\pm11.50$  & $-3.9\pm30.02$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
% & $1.4\pm0.59$   & $1.6\pm0.38$   & $1.6\pm0.37$   & $1.3\pm1.10$   & $0.5\pm1.55$    & $1.6\pm0.34$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\
% & $-1.3\pm13.36$ & $1.5\pm0.43$   & $1.6\pm0.37$   & $-4.7\pm23.79$ & $-13.1\pm66.30$ & $1.6\pm0.33$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\ \midrule
% & $ -2.9\pm 99.47$ & $  1.4\pm  3.08$ & $  1.6\pm  0.49$ & $-12.0\pm183.78$ & $-67.3\pm400.21$ &&& \\
% & $\B1.6\pm0.24$ & $\B1.6\pm0.17$ & $\B1.6\pm0.21$ & $\B1.6\pm0.42$ & $\B1.5\pm0.79$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.14$ \\
% & $1.0\pm2.38$   & $\B1.6\pm0.17$ & $\B1.6\pm0.21$ & $1.4\pm5.65$   & $-0.6\pm15.47$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.13$ \\
% & $1.6\pm0.39$   & $1.6\pm0.24$   & $1.6\pm0.25$   & $1.5\pm0.58$   & $1.1\pm1.25$    & $1.6\pm0.19$   & $1.6\pm0.12$   & $1.6\pm0.13$ \\
% & $-0.9\pm7.51$  & $1.6\pm0.23$   & $1.6\pm0.24$   & $-1.1\pm12.20$ & $-11.7\pm34.68$ & $\B1.6\pm0.18$ & $\R1.6\pm0.11$ & $\B1.6\pm0.12$ \\ \midrule
% & $-14.3\pm 60.88$ & $  0.8\pm  1.99$ & $  1.6\pm  0.31$ & $-14.7\pm132.57$ & $-95.5\pm264.74$ &&& \\
% & $\B1.6\pm0.18$ & $\B1.6\pm0.13$ & $\B1.6\pm0.14$ & $\B1.6\pm0.24$ & $\B1.6\pm0.44$  & $1.6\pm0.13$   & $1.6\pm0.09$   & $1.6\pm0.11$ \\
% & $1.6\pm1.34$   & $\B1.6\pm0.13$ & $\B1.6\pm0.14$ & $1.6\pm2.98$   & $1.6\pm6.06$    & $1.6\pm0.13$   & $1.7\pm0.09$   & $1.6\pm0.10$ \\
% & $\B1.6\pm0.18$ & $1.6\pm0.14$   & $1.6\pm0.16$   & $1.6\pm0.32$   & $1.5\pm0.74$    & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\
% & $0.5\pm3.15$   & $1.6\pm0.14$   & $1.6\pm0.16$   & $0.1\pm6.77$   & $-4.2\pm17.15$  & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\ \midrule
% & $-14.0\pm 42.91$ & $  1.2\pm  1.32$ & $  1.6\pm  0.24$ & $-27.9\pm 73.39$ & $-60.3\pm198.10$ &&& \\
% & $1.6\pm0.13$   & $1.6\pm0.10$   & $1.6\pm0.10$   & $\B1.6\pm0.17$ & $\B1.6\pm0.23$  & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
% & $1.6\pm0.64$   & $1.6\pm0.10$   & $1.6\pm0.10$   & $1.5\pm1.26$   & $1.3\pm2.98$    & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
% & $\B1.6\pm0.11$ & $\B1.6\pm0.08$ & $\B1.6\pm0.09$ & $\B1.6\pm0.17$ & $1.6\pm0.33$    & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $1.6\pm0.06$ \\
% & $1.2\pm1.32$   & $\B1.6\pm0.08$ & $\B1.6\pm0.09$ & $0.6\pm2.48$   & $-0.2\pm6.63$   & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $\B1.6\pm0.05$ \\


==> tab/pet-bf-par-sel-ja.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lllCCCC}
      \toprule
      \multicolumn{3}{l}{Proposal scales}  & \multicolumn{3}{c}{Manual} & Adaptive \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-7}
      \multicolumn{3}{l}{Annealing scheme} & Prior (5) & Posterior (5) & \multicolumn{2}{c}{Adaptive} \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-7}
      %
      $T$    & $N$   & Algorithm   & \multicolumn{4}{c}{Bayes factor estimates ($\log B_{2,1}\pm\text{\sd}$)} \\ \midrule
      $500$  & $30 $ & \pmcmc      & $1.7\pm0.62$ & $-70.9\pm525.79$ && \\
      $500$  & $192$ & \smctwo-\ds & $\B1.6\pm0.27$ & $\B1.3\pm1.13$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$  \\
             &       & \smctwo-\ps & $\B1.6\pm0.27$ & $-3.9\pm30.02$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$  \\
      $100 $ & $960$ & \smctwo-\ds & $1.6\pm0.37$   & $0.5\pm1.55$    & $1.6\pm0.34$   & $1.6\pm0.21$    \\
             &       & \smctwo-\ps & $1.6\pm0.37$   & $-13.1\pm66.30$ & $1.6\pm0.33$   & $1.6\pm0.21$    \\ \midrule
      $1000$ & $30 $ & \pmcmc      & $1.6\pm0.49$ & $-67.3\pm400.21$ && \\
      $1000$ & $192$ & \smctwo-\ds & $\B1.6\pm0.21$ & $\B1.5\pm0.79$  & $1.6\pm0.20$   & $1.6\pm0.13$   \\
             &       & \smctwo-\ps & $\B1.6\pm0.21$ & $-0.6\pm15.47$  & $1.6\pm0.20$   & $1.6\pm0.13$   \\
      $200 $ & $960$ & \smctwo-\ds & $1.6\pm0.25$   & $1.1\pm1.25$    & $1.6\pm0.19$   & $1.6\pm0.12$   \\
             &       & \smctwo-\ps & $1.6\pm0.24$   & $-11.7\pm34.68$ & $\B1.6\pm0.18$ & $\R1.6\pm0.11$ \\ \midrule
      $2000$ & $30 $ & \pmcmc      & $1.6\pm0.31$ & $-95.5\pm264.74$ && \\
      $2000$ & $192$ & \smctwo-\ds & $\B1.6\pm0.14$ & $\B1.6\pm0.44$  & $1.6\pm0.13$   & $1.6\pm0.09$    \\
             &       & \smctwo-\ps & $\B1.6\pm0.14$ & $1.6\pm6.06$    & $1.6\pm0.13$   & $1.7\pm0.09$    \\
      $400 $ & $960$ & \smctwo-\ds & $1.6\pm0.16$   & $1.5\pm0.74$    & $\B1.6\pm0.12$ & $\R1.6\pm0.08$  \\
             &       & \smctwo-\ps & $1.6\pm0.16$   & $-4.2\pm17.15$  & $\B1.6\pm0.12$ & $\R1.6\pm0.08$  \\ \midrule
      $5000$ & $30$  & \pmcmc      & $1.6\pm0.24$ & $-60.3\pm198.10$ && \\
      $5000$ & $192$ & \smctwo-\ds & $1.6\pm0.10$   & $\B1.6\pm0.23$  & $1.6\pm0.09$   & $1.6\pm0.05$    \\
             &       & \smctwo-\ps & $1.6\pm0.10$   & $1.3\pm2.98$    & $1.6\pm0.09$   & $1.6\pm0.05$    \\
      $1000$ & $960$ & \smctwo-\ds & $\B1.6\pm0.09$ & $1.6\pm0.33$    & $\B1.6\pm0.08$ & $\R1.6\pm0.04$  \\
             &       & \smctwo-\ps & $\B1.6\pm0.09$ & $-0.2\pm6.63$   & $\B1.6\pm0.08$ & $\R1.6\pm0.04$  \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Bayes factor $B_{2,1}$ estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. The \pmcmc and \smc with $N = 192$ are completely $N$-way
    parallelized.  \smc with $N = 960$ are $N/5$-way parallelized. {\B
      Italic}: Minimum variance for the same computational cost and the same schedule.
    {\R Bold}: Minimum variance for the same computational cost and all schedules.}
  \label{tab:pet-bf-par-sel}
\end{table}


% & $1.7\pm0.62$ & $-70.9\pm525.79$ &&& \\
% & $\B1.6\pm0.27$ & $\B1.3\pm1.13$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
% & $\B1.6\pm0.27$ & $-3.9\pm30.02$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
% & $1.6\pm0.37$   & $0.5\pm1.55$    & $1.6\pm0.34$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\
% & $1.6\pm0.37$   & $-13.1\pm66.30$ & $1.6\pm0.33$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\ \midrule
% & $1.6\pm0.49$ & $-67.3\pm400.21$ &&& \\
% & $\B1.6\pm0.21$ & $\B1.5\pm0.79$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.14$ \\
% & $\B1.6\pm0.21$ & $-0.6\pm15.47$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.13$ \\
% & $1.6\pm0.25$   & $1.1\pm1.25$    & $1.6\pm0.19$   & $1.6\pm0.12$   & $1.6\pm0.13$ \\
% & $1.6\pm0.24$   & $-11.7\pm34.68$ & $\B1.6\pm0.18$ & $\R1.6\pm0.11$ & $\B1.6\pm0.12$ \\ \midrule
% & $1.6\pm0.31$ & $-95.5\pm264.74$ &&& \\
% & $\B1.6\pm0.14$ & $\B1.6\pm0.44$  & $1.6\pm0.13$   & $1.6\pm0.09$   & $1.6\pm0.11$ \\
% & $\B1.6\pm0.14$ & $1.6\pm6.06$    & $1.6\pm0.13$   & $1.7\pm0.09$   & $1.6\pm0.10$ \\
% & $1.6\pm0.16$   & $1.5\pm0.74$    & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\
% & $1.6\pm0.16$   & $-4.2\pm17.15$  & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\ \midrule
% & $1.6\pm0.24$ & $-60.3\pm198.10$ &&& \\
% & $1.6\pm0.10$   & $\B1.6\pm0.23$  & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
% & $1.6\pm0.10$   & $1.3\pm2.98$    & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
% & $\B1.6\pm0.09$ & $1.6\pm0.33$    & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $1.6\pm0.06$ \\
% & $\B1.6\pm0.09$ & $-0.2\pm6.63$   & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $\B1.6\pm0.05$ \\


==> tab/pet-bf-par-sel.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lllCCCCC}
      \toprule
      \multicolumn{3}{l}{Proposal scales}  & \multicolumn{3}{c}{Manual} & Adaptive & Automatic \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}
      \multicolumn{3}{l}{Annealing scheme} & Prior (5) & Posterior (5) & \multicolumn{3}{c}{Adaptive} \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-8}
      %
      $T$    & $N$   & Algorithm   & \multicolumn{5}{c}{Bayes facor estimates ($\log B_{2,1}\pm\text{\sd}$)} \\ \midrule
      $500$  & $30 $ & \pmcmc      & $1.7\pm0.62$ & $-70.9\pm525.79$ &&& \\
      $500$  & $192$ & \smctwo-\ds & $\B1.6\pm0.27$ & $\B1.3\pm1.13$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
             &       & \smctwo-\ps & $\B1.6\pm0.27$ & $-3.9\pm30.02$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
      $100 $ & $960$ & \smctwo-\ds & $1.6\pm0.37$   & $0.5\pm1.55$    & $1.6\pm0.34$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\
             &       & \smctwo-\ps & $1.6\pm0.37$   & $-13.1\pm66.30$ & $1.6\pm0.33$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\ \midrule
      $1000$ & $30 $ & \pmcmc      & $1.6\pm0.49$ & $-67.3\pm400.21$ &&& \\
      $1000$ & $192$ & \smctwo-\ds & $\B1.6\pm0.21$ & $\B1.5\pm0.79$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.14$ \\
             &       & \smctwo-\ps & $\B1.6\pm0.21$ & $-0.6\pm15.47$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.13$ \\
      $200 $ & $960$ & \smctwo-\ds & $1.6\pm0.25$   & $1.1\pm1.25$    & $1.6\pm0.19$   & $1.6\pm0.12$   & $1.6\pm0.13$ \\
             &       & \smctwo-\ps & $1.6\pm0.24$   & $-11.7\pm34.68$ & $\B1.6\pm0.18$ & $\R1.6\pm0.11$ & $\B1.6\pm0.12$ \\ \midrule
      $2000$ & $30 $ & \pmcmc      & $1.6\pm0.31$ & $-95.5\pm264.74$ &&& \\
      $2000$ & $192$ & \smctwo-\ds & $\B1.6\pm0.14$ & $\B1.6\pm0.44$  & $1.6\pm0.13$   & $1.6\pm0.09$   & $1.6\pm0.11$ \\
             &       & \smctwo-\ps & $\B1.6\pm0.14$ & $1.6\pm6.06$    & $1.6\pm0.13$   & $1.7\pm0.09$   & $1.6\pm0.10$ \\
      $400 $ & $960$ & \smctwo-\ds & $1.6\pm0.16$   & $1.5\pm0.74$    & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\
             &       & \smctwo-\ps & $1.6\pm0.16$   & $-4.2\pm17.15$  & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\ \midrule
      $5000$ & $30$  & \pmcmc      & $1.6\pm0.24$ & $-60.3\pm198.10$ &&& \\
      $5000$ & $192$ & \smctwo-\ds & $1.6\pm0.10$   & $\B1.6\pm0.23$  & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
             &       & \smctwo-\ps & $1.6\pm0.10$   & $1.3\pm2.98$    & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
      $1000$ & $960$ & \smctwo-\ds & $\B1.6\pm0.09$ & $1.6\pm0.33$    & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $1.6\pm0.06$ \\
             &       & \smctwo-\ps & $\B1.6\pm0.09$ & $-0.2\pm6.63$   & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $\B1.6\pm0.05$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Bayes factor $B_{2,1}$ estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. The \pmcmc and \smc with $N = 192$ are completely $N$-way
    parallelized.  \smc with $N = 960$ are $N/5$-way parallelized. {\B
      Italic}: Best for the same computational cost and the same schedule.
    {\R Bold}: Best for the same computaitonal cost and all schedules.}
  \label{tab:pet-bf-par-sel}
\end{table}


% & $1.7\pm0.62$ & $-70.9\pm525.79$ &&& \\
% & $\B1.6\pm0.27$ & $\B1.3\pm1.13$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
% & $\B1.6\pm0.27$ & $-3.9\pm30.02$  & $\B1.6\pm0.20$ & $\R1.6\pm0.15$ & $\B1.6\pm0.16$ \\
% & $1.6\pm0.37$   & $0.5\pm1.55$    & $1.6\pm0.34$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\
% & $1.6\pm0.37$   & $-13.1\pm66.30$ & $1.6\pm0.33$   & $1.6\pm0.21$   & $1.6\pm0.17$ \\ \midrule
% & $1.6\pm0.49$ & $-67.3\pm400.21$ &&& \\
% & $\B1.6\pm0.21$ & $\B1.5\pm0.79$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.14$ \\
% & $\B1.6\pm0.21$ & $-0.6\pm15.47$  & $1.6\pm0.20$   & $1.6\pm0.13$   & $1.6\pm0.13$ \\
% & $1.6\pm0.25$   & $1.1\pm1.25$    & $1.6\pm0.19$   & $1.6\pm0.12$   & $1.6\pm0.13$ \\
% & $1.6\pm0.24$   & $-11.7\pm34.68$ & $\B1.6\pm0.18$ & $\R1.6\pm0.11$ & $\B1.6\pm0.12$ \\ \midrule
% & $1.6\pm0.31$ & $-95.5\pm264.74$ &&& \\
% & $\B1.6\pm0.14$ & $\B1.6\pm0.44$  & $1.6\pm0.13$   & $1.6\pm0.09$   & $1.6\pm0.11$ \\
% & $\B1.6\pm0.14$ & $1.6\pm6.06$    & $1.6\pm0.13$   & $1.7\pm0.09$   & $1.6\pm0.10$ \\
% & $1.6\pm0.16$   & $1.5\pm0.74$    & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\
% & $1.6\pm0.16$   & $-4.2\pm17.15$  & $\B1.6\pm0.12$ & $\R1.6\pm0.08$ & $\B1.6\pm0.09$ \\ \midrule
% & $1.6\pm0.24$ & $-60.3\pm198.10$ &&& \\
% & $1.6\pm0.10$   & $\B1.6\pm0.23$  & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
% & $1.6\pm0.10$   & $1.3\pm2.98$    & $1.6\pm0.09$   & $1.6\pm0.05$   & $1.6\pm0.06$ \\
% & $\B1.6\pm0.09$ & $1.6\pm0.33$    & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $1.6\pm0.06$ \\
% & $\B1.6\pm0.09$ & $-0.2\pm6.63$   & $\B1.6\pm0.08$ & $\R1.6\pm0.04$ & $\B1.6\pm0.05$ \\


==> tab/pet-bf-par.tex <==
\begin{table}
  \begingroup\small\begin{tabularx}{\textwidth}{lllXXXXl}
    \toprule
    &&& \multicolumn{5}{c}{Scheduler} \\
    \cmidrule(lr){4-8}
    $T$ & $N$ & Sampler & Linear & Prior & Posterior & Adaptive & $\overline{T}$ \\ \midrule
    $500 $ & $30 $ & \pmcmc      & $ -7.2\pm119.57$           & $1.7\pm0.64$             & $-88.9\pm437.10$             &                         & \\
    $500 $ & $192$ & \smctwo-\ds & $\color{blue}\it 1.6\pm0.39$   & $\color{red}\bf 1.6\pm0.30$  & $\color{blue}\it 1.1\pm1.22$     & $\color{red}\bf 1.6\pm0.30$ & $501$ \\
           &       & \smctwo-\ps & $  0.3\pm  6.36$           & $\color{red}\bf 1.6\pm0.30$  & $  2.0\pm 27.27$             & $1.6\pm0.32$            & \\
    $100 $ & $960$ & \smctwo-\ds & $  1.3\pm  0.69$           & $1.5\pm0.42$             & $  0.1\pm  1.95$             & $1.6\pm0.42$            & $104$ \\
           &       & \smctwo-\ps & $ -3.4\pm 11.90$           & $1.5\pm0.42$             & $-21.0\pm 62.19$             & $1.6\pm0.38$            & \\ \midrule
    $1000$ & $30 $ & \pmcmc      & $ -8.8\pm 65.96$           & $1.6\pm0.48$             & $-66.6\pm405.31$             &                         & \\
    $1000$ & $192$ & \smctwo-\ds & $\color{blue}\it 1.6\pm0.25$   & $\color{blue}\it 1.6\pm0.21$ & $\color{blue}\it 1.4\pm0.67$     & $1.6\pm0.18$            & $998$ \\
           &       & \smctwo-\ps & $  1.5\pm  2.72$           & $\color{blue}\it 1.6\pm0.21$ & $ -1.7\pm 15.88$             & $\color{red}\bf 1.6\pm0.17$ & \\
    $200 $ & $960$ & \smctwo-\ds & $  1.6\pm  0.36$           & $1.6\pm0.25$             & $  0.9\pm  1.14$             & $1.6\pm0.23$            & $216$ \\
           &       & \smctwo-\ps & $  0.0\pm  6.91$           & $1.6\pm0.25$             & $-12.0\pm 30.85$             & $1.6\pm0.24$            & \\ \midrule
    $2000$ & $30 $ & \pmcmc      & $-12.0\pm 59.59$           & $1.6\pm0.39$             & $-70.7\pm291.01$             &                         & \\
    $2000$ & $192$ & \smctwo-\ds & $\color{blue}\it 1.6\pm0.18$   & $1.7\pm0.15$             & $\color{blue}\it 1.6\pm0.38$     & $1.6\pm0.15$            & $1876$ \\
           &       & \smctwo-\ps & $  1.6\pm  1.48$           & $1.7\pm0.15$             & $  2.0\pm  8.29$             & $1.7\pm0.14$            & \\
    $400 $ & $960$ & \smctwo-\ds & $  1.6\pm  0.23$           & $\color{red}\bf 1.6\pm0.13$  & $  1.3\pm  0.79$             & $1.6\pm0.14$            & $388$ \\
           &       & \smctwo-\ps & $  0.4\pm  3.50$           & $\color{red}\bf 1.6\pm0.13$  & $ -6.7\pm 17.48$             & $\color{red}\bf 1.6\pm0.13$ & \\ \midrule
    $5000$ & $30 $ & \pmcmc      & $-13.7\pm 38.11$           & $1.6\pm0.25$             & $-58.3\pm183.15$             &                         & \\
    $5000$ & $192$ & \smctwo-\ds & $  1.6\pm  0.12$           & $1.6\pm0.08$             & $  \color{blue}\it 1.6\pm  0.23$ & $1.6\pm0.08$            & $4899$ \\
           &       & \smctwo-\ps & $  1.6\pm  0.63$           & $1.6\pm0.08$             & $  1.5\pm  2.79$             & $1.6\pm0.08$            & \\
    $1000$ & $960$ & \smctwo-\ds & $\color{blue}\it 1.6\pm  0.10$ & $\color{blue}\it 1.6\pm0.07$ & $  1.6\pm  0.35$             & $1.6\pm0.07$            & $972$ \\
           &       & \smctwo-\ps & $  0.7\pm  2.89$           & $\color{blue}\it 1.6\pm0.07$ & $  0.3\pm  5.72$             & $\color{red}\bf 1.6\pm0.06$ & \\
    \bottomrule
  \end{tabularx}\endgroup
  \caption{Bayes factor $B_{2,1}$ estimates of \pet model. $T$: Number of
    distributions in \smc and number of iterations used for inference in
    \pmcmc. $N$: Number of particles in \smc and number chains in \pmcmc.
    $\overline{T}$: The average number of time steps when using adaptive
    schedule.  
    The \pmcmc and \smc with $N = 192$ are completely $N$-way parallelized.
    \smc with $N = 960$ are $N/5$-way parallelized.  \textcolor{blue}{\it Italic}:
    Best for the same computational cost and the same schedule.
    \textcolor{red}{\bf Bold}: Best for the same computaitonal cost and all
    schedules.}
  \label{tab:pet-bf-par}
\end{table}


==> tab/pet-py-par-all.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lllCCCCCCCC}
      \toprule
      \multicolumn{3}{l}{Proposal scales}  & \multicolumn{6}{c}{Manual} & Adaptive & Automatic \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-9}\cmidrule(lr){10-10}\cmidrule(lr){11-11}
      \multicolumn{3}{l}{Annealing scheme} & Linear & Prior (2) & Prior (5) & Posterior (2) & Posterior (5) & \multicolumn{3}{c}{Adaptive} \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-11}
      %
      $T$    & $N$   & Algorithm   & \multicolumn{8}{c}{Marginal likelihood estimates ($\log p(\paramk|\data)\pm\text{\sd}$)} \\ \midrule
      $500$  & $30 $ & \pmcmc      & $-226.7\pm 86.34$ & $ -45.2\pm  2.52$ & $ -39.1\pm  0.56$ & $-407.5\pm168.17$ & $-926.8\pm376.99$ &&& \\
      $500$  & $192$ & \smctwo-\ds & $\B-39.2\pm0.30$ & $\B-39.2\pm0.25$ & $\B-39.2\pm0.25$ & $\B-39.5\pm0.57$ & $\B-39.7\pm1.06$ & $\B-39.2\pm0.18$ & $\R-39.1\pm0.12$ & $\B-39.2\pm0.13$ \\
             &       & \smctwo-\ps & $-50.0\pm4.86$   & $\B-39.2\pm0.25$ & $\B-39.2\pm0.25$ & $-60.5\pm8.74$   & $-91.3\pm21.69$  & $\B-39.2\pm0.18$ & $-39.1\pm0.13$   & $\B-39.2\pm0.13$ \\
      $100 $ & $960$ & \smctwo-\ds & $-39.5\pm0.57$   & $-39.2\pm0.37$   & $-39.3\pm0.36$   & $-39.7\pm1.08$   & $-40.6\pm1.41$   & $-39.2\pm0.31$   & $-39.2\pm0.19$   & $-39.2\pm0.18$ \\
             &       & \smctwo-\ps & $-92.5\pm10.02$  & $-39.7\pm0.40$   & $-39.3\pm0.35$   & $145.8\pm17.86$  & $302.1\pm46.29$  & $-39.3\pm0.31$   & $-39.2\pm0.18$   & $-39.2\pm0.19$ \\ \midrule
      $1000$ & $30 $ & \pmcmc      & $-218.9\pm 60.53$ & $ -45.3\pm  2.46$ & $ -39.3\pm  0.46$ & $-402.1\pm117.18$ & $-884.1\pm307.88$ &&& \\
      $1000$ & $192$ & \smctwo-\ds & $\B-39.2\pm0.21$ & $\B-39.2\pm0.15$ & $\B-39.2\pm0.19$ & $\B-39.2\pm0.37$ & $\B-39.4\pm0.68$ & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $-39.2\pm0.11$ \\
             &       & \smctwo-\ps & $-44.4\pm2.11$   & $\B-39.2\pm0.15$ & $\B-39.2\pm0.19$ & $-49.3\pm4.29$   & $-66.0\pm13.26$  & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $\R-39.2\pm0.10$ \\
      $200 $ & $960$ & \smctwo-\ds & $-39.2\pm0.37$   & $-39.2\pm0.21$   & $-39.2\pm0.22$   & $-39.4\pm0.54$   & $-39.8\pm1.21$   & $-39.2\pm0.18$   & $-39.1\pm0.11$   & $-39.2\pm0.11$ \\
             &       & \smctwo-\ps & $-66.0\pm5.10$   & $-39.3\pm0.20$   & $-39.2\pm0.22$   & $-90.9\pm7.84$   & $175.5\pm26.84$  & $-39.2\pm0.18$   & $-39.2\pm0.11$   & $-39.2\pm0.12$ \\ \midrule
      $2000$ & $30 $ & \pmcmc      & $-225.7\pm 43.83$ & $ -45.5\pm  1.58$ & $ -39.3\pm  0.28$ & $-407.0\pm 90.41$ & $-928.7\pm204.93$ &&& \\
      $2000$ & $192$ & \smctwo-\ds & $\B-39.1\pm0.15$ & $-39.2\pm0.13$   & $-39.2\pm0.14$   & $\B-39.2\pm0.21$ & $\B-39.3\pm0.41$ & $-39.1\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
             &       & \smctwo-\ps & $-41.5\pm1.02$   & $-39.2\pm0.13$   & $-39.2\pm0.14$   & $-44.2\pm2.18$   & $-51.2\pm4.30$   & $-39.2\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
      $400 $ & $960$ & \smctwo-\ds & $-39.2\pm0.18$   & $\B-39.2\pm0.12$ & $\B-39.2\pm0.13$ & $-39.2\pm0.31$   & $-39.4\pm0.73$   & $\B-39.2\pm0.11$ & $-39.2\pm0.07$   & $-39.2\pm0.08$ \\
             &       & \smctwo-\ps & $-52.2\pm2.40$   & $\B-39.2\pm0.12$ & $\B-39.2\pm0.13$ & $-65.6\pm4.83$   & $106.0\pm14.36$  & $\B-39.2\pm0.11$ & $\R-39.2\pm0.06$ & $-39.2\pm0.08$ \\ \midrule
      $5000$ & $30$  & \pmcmc      & $-227.3\pm 33.66$ & $ -45.3\pm  0.98$ & $ -39.3\pm  0.21$ & $-408.9\pm 51.78$ & $-917.6\pm129.54$ &&& \\
      $5000$ & $192$ & \smctwo-\ds & $-39.2\pm0.10$   & $-39.2\pm0.09$   & $-39.2\pm0.09$   & $\B-39.2\pm0.14$ & $\B-39.2\pm0.20$ & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.05$ \\
             &       & \smctwo-\ps & $-40.1\pm0.44$   & $-39.2\pm0.09$   & $-39.2\pm0.09$   & $-41.1\pm0.75$   & $-43.8\pm2.13$   & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.04$ \\
      $1000$ & $960$ & \smctwo-\ds & $\B-39.2\pm0.09$ & $\B-39.2\pm0.06$ & $\B-39.2\pm0.08$ & $-39.2\pm0.16$   & $-39.2\pm0.31$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $-39.2\pm0.06$ \\
             &       & \smctwo-\ps & $-44.4\pm1.02$   & $-39.2\pm0.07$   & $\B-39.2\pm0.08$ & $-49.7\pm1.99$   & $-65.7\pm5.54$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $\B-39.2\pm0.04$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Marginal likelihood estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. The \pmcmc and \smc with $N = 192$ are completely $N$-way
    parallelized.  \smc with $N = 960$ are $N/5$-way parallelized. {\B
      Italic}: Best for the same computational cost and the same proposal
    scales and annealing schemes.  {\R Bold}: Best for the same computaitonal
    cost and all proposal scales and annealing schemes.}
  \label{tab:pet-py-par-all}
\end{table}

% & $-226.7\pm 86.34$ & $ -45.2\pm  2.52$ & $ -39.1\pm  0.56$ & $-407.5\pm168.17$ & $-926.8\pm376.99$ &&& \\
% & $\B-39.2\pm0.30$ & $\B-39.2\pm0.25$ & $\B-39.2\pm0.25$ & $\B-39.5\pm0.57$ & $\B-39.7\pm1.06$ & $\B-39.2\pm0.18$ & $\R-39.1\pm0.12$ & $\B-39.2\pm0.13$ \\
% & $-50.0\pm4.86$   & $\B-39.2\pm0.25$ & $\B-39.2\pm0.25$ & $-60.5\pm8.74$   & $-91.3\pm21.69$  & $\B-39.2\pm0.18$ & $-39.1\pm0.13$   & $\B-39.2\pm0.13$ \\
% & $-39.5\pm0.57$   & $-39.2\pm0.37$   & $-39.3\pm0.36$   & $-39.7\pm1.08$   & $-40.6\pm1.41$   & $-39.2\pm0.31$   & $-39.2\pm0.19$   & $-39.2\pm0.18$ \\
% & $-92.5\pm10.02$  & $-39.7\pm0.40$   & $-39.3\pm0.35$   & $145.8\pm17.86$  & $302.1\pm46.29$  & $-39.3\pm0.31$   & $-39.2\pm0.18$   & $-39.2\pm0.19$ \\ \midrule
% & $-218.9\pm 60.53$ & $ -45.3\pm  2.46$ & $ -39.3\pm  0.46$ & $-402.1\pm117.18$ & $-884.1\pm307.88$ &&& \\
% & $\B-39.2\pm0.21$ & $\B-39.2\pm0.15$ & $\B-39.2\pm0.19$ & $\B-39.2\pm0.37$ & $\B-39.4\pm0.68$ & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $-39.2\pm0.11$ \\
% & $-44.4\pm2.11$   & $\B-39.2\pm0.15$ & $\B-39.2\pm0.19$ & $-49.3\pm4.29$   & $-66.0\pm13.26$  & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $\R-39.2\pm0.10$ \\
% & $-39.2\pm0.37$   & $-39.2\pm0.21$   & $-39.2\pm0.22$   & $-39.4\pm0.54$   & $-39.8\pm1.21$   & $-39.2\pm0.18$   & $-39.1\pm0.11$   & $-39.2\pm0.11$ \\
% & $-66.0\pm5.10$   & $-39.3\pm0.20$   & $-39.2\pm0.22$   & $-90.9\pm7.84$   & $175.5\pm26.84$  & $-39.2\pm0.18$   & $-39.2\pm0.11$   & $-39.2\pm0.12$ \\ \midrule
% & $-225.7\pm 43.83$ & $ -45.5\pm  1.58$ & $ -39.3\pm  0.28$ & $-407.0\pm 90.41$ & $-928.7\pm204.93$ &&& \\
% & $\B-39.1\pm0.15$ & $-39.2\pm0.13$   & $-39.2\pm0.14$   & $\B-39.2\pm0.21$ & $\B-39.3\pm0.41$ & $-39.1\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
% & $-41.5\pm1.02$   & $-39.2\pm0.13$   & $-39.2\pm0.14$   & $-44.2\pm2.18$   & $-51.2\pm4.30$   & $-39.2\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
% & $-39.2\pm0.18$   & $\B-39.2\pm0.12$ & $\B-39.2\pm0.13$ & $-39.2\pm0.31$   & $-39.4\pm0.73$   & $\B-39.2\pm0.11$ & $-39.2\pm0.07$   & $-39.2\pm0.08$ \\
% & $-52.2\pm2.40$   & $\B-39.2\pm0.12$ & $\B-39.2\pm0.13$ & $-65.6\pm4.83$   & $106.0\pm14.36$  & $\B-39.2\pm0.11$ & $\R-39.2\pm0.06$ & $-39.2\pm0.08$ \\ \midrule
% & $-227.3\pm 33.66$ & $ -45.3\pm  0.98$ & $ -39.3\pm  0.21$ & $-408.9\pm 51.78$ & $-917.6\pm129.54$ &&& \\
% & $-39.2\pm0.10$   & $-39.2\pm0.09$   & $-39.2\pm0.09$   & $\B-39.2\pm0.14$ & $\B-39.2\pm0.20$ & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.05$ \\
% & $-40.1\pm0.44$   & $-39.2\pm0.09$   & $-39.2\pm0.09$   & $-41.1\pm0.75$   & $-43.8\pm2.13$   & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.04$ \\
% & $\B-39.2\pm0.09$ & $\B-39.2\pm0.06$ & $\B-39.2\pm0.08$ & $-39.2\pm0.16$   & $-39.2\pm0.31$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $-39.2\pm0.06$ \\
% & $-44.4\pm1.02$   & $-39.2\pm0.07$   & $\B-39.2\pm0.08$ & $-49.7\pm1.99$   & $-65.7\pm5.54$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $\B-39.2\pm0.04$ \\


==> tab/pet-py-par-sel-ja.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lllCCCC}
      \toprule
      \multicolumn{3}{l}{Proposal scales}  & \multicolumn{3}{c}{Manual} & Adaptive \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-7}
      \multicolumn{3}{l}{Annealing scheme} & Prior (5) & Posterior (5) & \multicolumn{2}{c}{Adaptive} \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-7}
      %
      $T$    & $N$   & Algorithm   & \multicolumn{4}{c}{Marginal likelihood estimates ($\log p(\data|\Mk)\pm\text{\sd}$)} \\ \midrule
      $500$  & $30 $ & \pmcmc      & $ -39.1\pm  0.56$ & $-926.8\pm376.99$ && \\
      $500$  & $192$ & \smctwo-\ds & $\B-39.2\pm0.25$ & $\B-39.7\pm1.06$ & $\B-39.2\pm0.18$ & $\R-39.1\pm0.12$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.25$ & $-91.3\pm21.69$  & $\B-39.2\pm0.18$ & $-39.1\pm0.13$   \\
      $100 $ & $960$ & \smctwo-\ds & $-39.3\pm0.36$   & $-40.6\pm1.41$   & $-39.2\pm0.31$   & $-39.2\pm0.19$   \\
             &       & \smctwo-\ps & $-39.3\pm0.35$   & $302.1\pm46.29$  & $-39.3\pm0.31$   & $-39.2\pm0.18$   \\ \midrule
      $1000$ & $30 $ & \pmcmc      & $ -39.3\pm  0.46$ & $-884.1\pm307.88$ && \\
      $1000$ & $192$ & \smctwo-\ds & $\B-39.2\pm0.19$ & $\B-39.4\pm0.68$ & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.19$ & $-66.0\pm13.26$  & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$  \\
      $200 $ & $960$ & \smctwo-\ds & $-39.2\pm0.22$   & $-39.8\pm1.21$   & $-39.2\pm0.18$   & $-39.1\pm0.11$   \\
             &       & \smctwo-\ps & $-39.2\pm0.22$   & $175.5\pm26.84$  & $-39.2\pm0.18$   & $-39.2\pm0.11$   \\ \midrule
      $2000$ & $30 $ & \pmcmc      & $ -39.3\pm  0.28$ & $-928.7\pm204.93$ && \\
      $2000$ & $192$ & \smctwo-\ds & $-39.2\pm0.14$   & $\B-39.3\pm0.41$ & $-39.1\pm0.12$   & $-39.1\pm0.07$  \\
             &       & \smctwo-\ps & $-39.2\pm0.14$   & $-51.2\pm4.30$   & $-39.2\pm0.12$   & $-39.1\pm0.07$  \\
      $400 $ & $960$ & \smctwo-\ds & $\B-39.2\pm0.13$ & $-39.4\pm0.73$   & $\B-39.2\pm0.11$ & $-39.2\pm0.07$   \\
             &       & \smctwo-\ps & $\B-39.2\pm0.13$ & $106.0\pm14.36$  & $\B-39.2\pm0.11$ & $\R-39.2\pm0.06$ \\ \midrule
      $5000$ & $30$  & \pmcmc      & $ -39.3\pm  0.21$ & $-917.6\pm129.54$ && \\
      $5000$ & $192$ & \smctwo-\ds & $-39.2\pm0.09$   & $\B-39.2\pm0.20$ & $-39.2\pm0.08$   & $-39.1\pm0.04$   \\
             &       & \smctwo-\ps & $-39.2\pm0.09$   & $-43.8\pm2.13$   & $-39.2\pm0.08$   & $-39.1\pm0.04$   \\
      $1000$ & $960$ & \smctwo-\ds & $\B-39.2\pm0.08$ & $-39.2\pm0.31$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.08$ & $-65.7\pm5.54$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Marginal likelihood estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. The \pmcmc and \smc with $N = 192$ are completely $N$-way
    parallelized.  \smc with $N = 960$ are $N/5$-way parallelized. {\B
      Italic}: Minimum variance for the same computational cost and the same proposal
    scales and annealing schemes.  {\R Bold}: Minimum variance for the same computaitonal
    cost and all proposal scales and annealing schemes.}
  \label{tab:pet-py-par-sel}
\end{table}

% & & $ -39.1\pm  0.56$ & $-926.8\pm376.99$ &&& \\
% & $\B-39.2\pm0.25$ & $\B-39.7\pm1.06$ & $\B-39.2\pm0.18$ & $\R-39.1\pm0.12$ & $\B-39.2\pm0.13$ \\
% & $\B-39.2\pm0.25$ & $-91.3\pm21.69$  & $\B-39.2\pm0.18$ & $-39.1\pm0.13$   & $\B-39.2\pm0.13$ \\
% & $-39.3\pm0.36$   & $-40.6\pm1.41$   & $-39.2\pm0.31$   & $-39.2\pm0.19$   & $-39.2\pm0.18$ \\
% & $-39.3\pm0.35$   & $302.1\pm46.29$  & $-39.3\pm0.31$   & $-39.2\pm0.18$   & $-39.2\pm0.19$ \\ \midrule
% & & $ -39.3\pm  0.46$ & $-884.1\pm307.88$ &&& \\
% & $\B-39.2\pm0.19$ & $\B-39.4\pm0.68$ & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $-39.2\pm0.11$ \\
% & $\B-39.2\pm0.19$ & $-66.0\pm13.26$  & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $\R-39.2\pm0.10$ \\
% & $-39.2\pm0.22$   & $-39.8\pm1.21$   & $-39.2\pm0.18$   & $-39.1\pm0.11$   & $-39.2\pm0.11$ \\
% & $-39.2\pm0.22$   & $175.5\pm26.84$  & $-39.2\pm0.18$   & $-39.2\pm0.11$   & $-39.2\pm0.12$ \\ \midrule
% & & $ -39.3\pm  0.28$ & $-928.7\pm204.93$ &&& \\
% & $-39.2\pm0.14$   & $\B-39.3\pm0.41$ & $-39.1\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
% & $-39.2\pm0.14$   & $-51.2\pm4.30$   & $-39.2\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
% & $\B-39.2\pm0.13$ & $-39.4\pm0.73$   & $\B-39.2\pm0.11$ & $-39.2\pm0.07$   & $-39.2\pm0.08$ \\
% & $\B-39.2\pm0.13$ & $106.0\pm14.36$  & $\B-39.2\pm0.11$ & $\R-39.2\pm0.06$ & $-39.2\pm0.08$ \\ \midrule
% & & $ -39.3\pm  0.21$ & $-917.6\pm129.54$ &&& \\
% & $-39.2\pm0.09$   & $\B-39.2\pm0.20$ & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.05$ \\
% & $-39.2\pm0.09$   & $-43.8\pm2.13$   & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.04$ \\
% & $\B-39.2\pm0.08$ & $-39.2\pm0.31$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $-39.2\pm0.06$ \\
% & $\B-39.2\pm0.08$ & $-65.7\pm5.54$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $\B-39.2\pm0.04$ \\


==> tab/pet-py-par-sel.tex <==
\begin{table}
  \def\B{\color{blue}\it}
  \def\R{\color{red}\bf}
  \begingroup\small
    \begin{tabularx}{\linewidth}{lllCCCCC}
      \toprule
      \multicolumn{3}{l}{Proposal scales}  & \multicolumn{3}{c}{Manual} & Adaptive & Automatic \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}
      \multicolumn{3}{l}{Annealing scheme} & Prior (5) & Posterior (5) & \multicolumn{3}{c}{Adaptive} \\
      \cmidrule(lr){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-8}
      %
      $T$    & $N$   & Algorithm   & \multicolumn{5}{c}{Marginal likelihood estimates ($\log p(\paramk|\data)\pm\text{\sd}$)} \\ \midrule
      $500$  & $30 $ & \pmcmc      & $ -39.1\pm  0.56$ & $-926.8\pm376.99$ &&& \\
      $500$  & $192$ & \smctwo-\ds & $\B-39.2\pm0.25$ & $\B-39.7\pm1.06$ & $\B-39.2\pm0.18$ & $\R-39.1\pm0.12$ & $\B-39.2\pm0.13$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.25$ & $-91.3\pm21.69$  & $\B-39.2\pm0.18$ & $-39.1\pm0.13$   & $\B-39.2\pm0.13$ \\
      $100 $ & $960$ & \smctwo-\ds & $-39.3\pm0.36$   & $-40.6\pm1.41$   & $-39.2\pm0.31$   & $-39.2\pm0.19$   & $-39.2\pm0.18$ \\
             &       & \smctwo-\ps & $-39.3\pm0.35$   & $302.1\pm46.29$  & $-39.3\pm0.31$   & $-39.2\pm0.18$   & $-39.2\pm0.19$ \\ \midrule
      $1000$ & $30 $ & \pmcmc      & $ -39.3\pm  0.46$ & $-884.1\pm307.88$ &&& \\
      $1000$ & $192$ & \smctwo-\ds & $\B-39.2\pm0.19$ & $\B-39.4\pm0.68$ & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $-39.2\pm0.11$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.19$ & $-66.0\pm13.26$  & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $\R-39.2\pm0.10$ \\
      $200 $ & $960$ & \smctwo-\ds & $-39.2\pm0.22$   & $-39.8\pm1.21$   & $-39.2\pm0.18$   & $-39.1\pm0.11$   & $-39.2\pm0.11$ \\
             &       & \smctwo-\ps & $-39.2\pm0.22$   & $175.5\pm26.84$  & $-39.2\pm0.18$   & $-39.2\pm0.11$   & $-39.2\pm0.12$ \\ \midrule
      $2000$ & $30 $ & \pmcmc      & $ -39.3\pm  0.28$ & $-928.7\pm204.93$ &&& \\
      $2000$ & $192$ & \smctwo-\ds & $-39.2\pm0.14$   & $\B-39.3\pm0.41$ & $-39.1\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
             &       & \smctwo-\ps & $-39.2\pm0.14$   & $-51.2\pm4.30$   & $-39.2\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
      $400 $ & $960$ & \smctwo-\ds & $\B-39.2\pm0.13$ & $-39.4\pm0.73$   & $\B-39.2\pm0.11$ & $-39.2\pm0.07$   & $-39.2\pm0.08$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.13$ & $106.0\pm14.36$  & $\B-39.2\pm0.11$ & $\R-39.2\pm0.06$ & $-39.2\pm0.08$ \\ \midrule
      $5000$ & $30$  & \pmcmc      & $ -39.3\pm  0.21$ & $-917.6\pm129.54$ &&& \\
      $5000$ & $192$ & \smctwo-\ds & $-39.2\pm0.09$   & $\B-39.2\pm0.20$ & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.05$ \\
             &       & \smctwo-\ps & $-39.2\pm0.09$   & $-43.8\pm2.13$   & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.04$ \\
      $1000$ & $960$ & \smctwo-\ds & $\B-39.2\pm0.08$ & $-39.2\pm0.31$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $-39.2\pm0.06$ \\
             &       & \smctwo-\ps & $\B-39.2\pm0.08$ & $-65.7\pm5.54$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $\B-39.2\pm0.04$ \\
      \bottomrule
    \end{tabularx}
  \endgroup
  \caption{Marginal likelihood estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. The \pmcmc and \smc with $N = 192$ are completely $N$-way
    parallelized.  \smc with $N = 960$ are $N/5$-way parallelized. {\B
      Italic}: Best for the same computational cost and the same proposal
    scales and annealing schemes.  {\R Bold}: Best for the same computaitonal
    cost and all proposal scales and annealing schemes.}
  \label{tab:pet-py-par-sel}
\end{table}

% & & $ -39.1\pm  0.56$ & $-926.8\pm376.99$ &&& \\
% & $\B-39.2\pm0.25$ & $\B-39.7\pm1.06$ & $\B-39.2\pm0.18$ & $\R-39.1\pm0.12$ & $\B-39.2\pm0.13$ \\
% & $\B-39.2\pm0.25$ & $-91.3\pm21.69$  & $\B-39.2\pm0.18$ & $-39.1\pm0.13$   & $\B-39.2\pm0.13$ \\
% & $-39.3\pm0.36$   & $-40.6\pm1.41$   & $-39.2\pm0.31$   & $-39.2\pm0.19$   & $-39.2\pm0.18$ \\
% & $-39.3\pm0.35$   & $302.1\pm46.29$  & $-39.3\pm0.31$   & $-39.2\pm0.18$   & $-39.2\pm0.19$ \\ \midrule
% & & $ -39.3\pm  0.46$ & $-884.1\pm307.88$ &&& \\
% & $\B-39.2\pm0.19$ & $\B-39.4\pm0.68$ & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $-39.2\pm0.11$ \\
% & $\B-39.2\pm0.19$ & $-66.0\pm13.26$  & $\B-39.2\pm0.17$ & $\R-39.1\pm0.10$ & $\R-39.2\pm0.10$ \\
% & $-39.2\pm0.22$   & $-39.8\pm1.21$   & $-39.2\pm0.18$   & $-39.1\pm0.11$   & $-39.2\pm0.11$ \\
% & $-39.2\pm0.22$   & $175.5\pm26.84$  & $-39.2\pm0.18$   & $-39.2\pm0.11$   & $-39.2\pm0.12$ \\ \midrule
% & & $ -39.3\pm  0.28$ & $-928.7\pm204.93$ &&& \\
% & $-39.2\pm0.14$   & $\B-39.3\pm0.41$ & $-39.1\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
% & $-39.2\pm0.14$   & $-51.2\pm4.30$   & $-39.2\pm0.12$   & $-39.1\pm0.07$   & $\B-39.2\pm0.07$ \\
% & $\B-39.2\pm0.13$ & $-39.4\pm0.73$   & $\B-39.2\pm0.11$ & $-39.2\pm0.07$   & $-39.2\pm0.08$ \\
% & $\B-39.2\pm0.13$ & $106.0\pm14.36$  & $\B-39.2\pm0.11$ & $\R-39.2\pm0.06$ & $-39.2\pm0.08$ \\ \midrule
% & & $ -39.3\pm  0.21$ & $-917.6\pm129.54$ &&& \\
% & $-39.2\pm0.09$   & $\B-39.2\pm0.20$ & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.05$ \\
% & $-39.2\pm0.09$   & $-43.8\pm2.13$   & $-39.2\pm0.08$   & $-39.1\pm0.04$   & $-39.1\pm0.04$ \\
% & $\B-39.2\pm0.08$ & $-39.2\pm0.31$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $-39.2\pm0.06$ \\
% & $\B-39.2\pm0.08$ & $-65.7\pm5.54$   & $\B-39.2\pm0.07$ & $\R-39.2\pm0.03$ & $\B-39.2\pm0.04$ \\


==> tab/pet-py-par.tex <==
\begin{table}
  \begingroup\small\begin{tabularx}{\textwidth}{lllXXXXl}
    \toprule
    &&& \multicolumn{5}{c}{Scheduler} \\
    \cmidrule(lr){4-8}
    $T$ & $N$ & Sampler & Linear & Prior & Posterior & Adaptive & $\overline{T}$ \\ \midrule
    $500$  & $30 $ & \pmcmc      & $-214.6\pm84.37$            & $-39.3\pm0.62$             & $-920.3\pm359.21$          &                            & \\
    $500$  & $192$ & \smctwo-\ds & $\color{blue}\it -39.2\pm0.33$  & $\color{red}\bf -39.1\pm0.27$  & $\color{blue}\it -39.9\pm1.13$ & $-39.2\pm0.39$             & $487$ \\
           &       & \smctwo-\ps & $ -49.9\pm 4.47$            & $\color{red}\bf -39.1\pm0.27$  & $ -88.8\pm 17.40$          & $\color{blue}\it -39.0\pm0.38$ & \\
    $100 $ & $960$ & \smctwo-\ds & $ -39.5\pm 0.66$            & $-39.2\pm0.41$             & $ -41.0\pm  1.72$          & $-39.1\pm0.61$             & $86$ \\
           &       & \smctwo-\ps & $ -92.2\pm 9.05$            & $-39.2\pm0.40$             & $-307.0\pm 43.73$          & $-39.1\pm0.58$             & \\ \midrule
    $1000$ & $30 $ & \pmcmc      & $-215.5\pm48.81$            & $-39.3\pm0.45$             & $-901.4\pm287.39$          &                            & \\
    $1000$ & $192$ & \smctwo-\ds & $\color{blue}\it -39.2\pm 0.21$ & $\color{red}\bf -39.1\pm0.20$  & $\color{blue}\it -39.4\pm0.62$ & $\color{blue}\it -39.1\pm0.30$ & $978$ \\
           &       & \smctwo-\ps & $ -44.3\pm 1.87$            & $\color{red}\bf -39.1\pm0.20$  & $ -65.6\pm 12.85$          & $-39.1\pm0.31$             & \\
    $200 $ & $960$ & \smctwo-\ds & $ -39.2\pm 0.34$            & $-39.2\pm0.23$             & $ -40.0\pm  1.05$          & $-39.3\pm0.43$             & $206$ \\
           &       & \smctwo-\ps & $ -65.4\pm 4.79$            & $-39.2\pm0.23$             & $-175.2\pm 23.16$          & $-39.2\pm0.42$             & \\ \midrule
    $2000$ & $30 $ & \pmcmc      & $-226.2\pm46.20$            & $-39.3\pm0.35$             & $-919.9\pm203.52$          &                            & \\
    $2000$ & $192$ & \smctwo-\ds & $\color{blue}\it -39.1\pm 0.15$ & $-39.1\pm0.14$             & $\color{blue}\it -39.2\pm0.35$ & $-39.1\pm0.15$             & $1967$ \\
           &       & \smctwo-\ps & $ -41.5\pm 1.01$            & $-39.1\pm0.14$             & $ -51.8\pm  4.61$          & $-39.1\pm0.14$             & \\
    $400 $ & $960$ & \smctwo-\ds & $ -39.2\pm 0.21$            & $\color{red}\bf -39.1\pm0.13$  & $ -39.5\pm  0.72$          & $-39.0\pm0.14$             & $378$ \\
           &       & \smctwo-\ps & $ -52.4\pm 2.65$            & $\color{red}\bf -39.1\pm0.13$  & $-106.7\pm 12.19$          & $\color{red}\bf -39.1\pm0.13$  & \\ \midrule
    $5000$ & $30$  & \pmcmc      & $-225.1\pm26.06$            & $-39.3\pm0.24$             & $-905.9\pm122.63$          &                            & \\
    $5000$ & $192$ & \smctwo-\ds & $ -39.2\pm 0.09$            & $\color{blue}\it -39.1\pm0.07$ & $ -39.2\pm  0.19$          & $-39.1\pm0.05$             & $4589$ \\
           &       & \smctwo-\ps & $ -40.0\pm 0.46$            & $\color{blue}\it -39.1\pm0.07$ & $ -44.2\pm  2.12$          & $-39.1\pm0.05$             & \\
    $1000$ & $960$ & \smctwo-\ds & $\color{blue}\it -39.1\pm 0.08$ & $\color{blue}\it -39.2\pm0.07$ & $\color{blue}\it -39.2\pm0.32$ & $-39.2\pm0.04$             & $981$ \\
           &       & \smctwo-\ps & $ -44.6\pm 2.73$            & $-39.2\pm0.07$             & $ -64.9\pm  4.68$          & $\color{red}\bf -39.1\pm0.03$  & \\
    \bottomrule
  \end{tabularx}\endgroup
  \caption{Marginal likelihood estimates of two components \pet model. $T$:
    Number of distributions in \smc and number of iterations used for
    inference in \pmcmc. $N$: Number of particles in \smc and number chains in
    \pmcmc. $\overline{T}$: The average number of time steps when using
    adaptive schedule.
    The \pmcmc and \smc with $N = 192$ are completely $N$-way parallelized.
    \smc with $N = 960$ are $N/5$-way parallelized.  \textcolor{blue}{\it Italic}:
    Best for the same computational cost and the same schedule.
    \textcolor{red}{\bf Bold}: Best for the same computaitonal cost and all
    schedules.}
  \label{tab:pet-py-par}
\end{table}

